Adaptive Periodic Averaging: A Practical Approach to Reducing Communication in Distributed Learning

Stochastic Gradient Descent (SGD) is the key learning algorithm for many machine learning tasks. Because of its computational costs, there is a growing interest in accelerating SGD on HPC resources like GPU clusters. However, the performance of parallel SGD is still bottlenecked by the high communication costs even with a fast connection among the machines. A simple approach to alleviating this problem, used in many existing efforts, is to perform communication every few iterations, using a constant averaging period. In this paper, we show that the optimal averaging period in terms of convergence and communication cost is not a constant, but instead varies over the course of the execution. Specifically, we observe that reducing the variance of model parameters among the computing nodes is critical to the convergence of periodic parameter averaging SGD. Given a fixed communication budget, we show that it is more beneficial to synchronize more frequently in early iterations to reduce the initial large variance and synchronize less frequently in the later phase of the training process. We propose a practical algorithm, named ADaptive Periodic parameter averaging SGD (ADPSGD), to achieve a smaller overall variance of model parameters, and thus better convergence compared with the Constant Periodic parameter averaging SGD (CPSGD). We evaluate our method with several image classification benchmarks and show that our ADPSGD indeed achieves smaller training losses and higher test accuracies with smaller communication compared with CPSGD. Compared with gradient-quantization SGD, we show that our algorithm achieves faster convergence with only half of the communication. Compared with full-communication SGD, our ADPSGD achieves 1:14x to 1:27x speedups with a 100Gbps connection among computing nodes, and the speedups increase to 1:46x ~ 1:95x with a 10Gbps connection.

==> figures/tmp-pdfcrop-13950.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{76676731362D31365F74696D652E706466}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfoutput=1 %
\pdfcompresslevel=9 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1<5 %
      \pdfobjcompresslevel=0 %
    \else
      \pdfobjcompresslevel=2 %
    \fi
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#1\relax
    }%
  }{%
    \pdfminorversion=#1\relax
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{4}
\page 1 [19 25 483 339]
\csname @@end\endcsname
\end


==> text/proofs.tex <==
\normalsize
\appendix
\pagenumbering{gobble}

\onecolumn


\normalsize
\appendix
\pagenumbering{gobble}

\onecolumn
\section{Derivation of (\ref{eq:step8})}
First, because $A_n\dotavg{n}=\dotavg{n}$, we have:
\begin{equation}
\label{eq:step1}
	\mathbb{E}f\myparam{W_{k+1}\dotavg{n}} = \mathbb{E}f\myparam{W_k\dotavg{n}-\gamma_k G(W_k;B_k)\dotavg{n}}.
\end{equation}
Then, we apply Lipschitzan gradient assumption to (\ref{eq:step1}) and obtain: 
\begin{flalign}
\label{eq:step2}
	\mathbb{E}f\myparam{W_k\dotavg{n}-\gamma_k G(W_k;B_k)\dotavg{n}}  \leq \mathbb{E} f\myparam{W_{k}\dotavg{n}}  - \gamma_k \mathbb{E}\myrect{ \nabla f\myparam{W_k\dotavg{n}}^T  \myparam{G\myparam{W_k;B_k}\dotavg{n}}}
	+ \frac{L\gamma_k^2}{2}\mathbb{E}\norm{G(W_k;B_k)\dotavg{n}}, 
\end{flalign}
where $L>0$ is the Lipschitz constant of the objective function. 
Next, we assume the stochastic gradients are unbiased, we have:
 \begin{flalign}
\label{eq:step3}
\mathbb{E}\myrect{ \nabla f\myparam{W_k\dotavg{n}}^T  \myparam{G\myparam{W_k;B_k}\dotavg{n}}} = \mathbb{E}\myrect{ \nabla f\myparam{W_k\dotavg{n}}^T  \myparam{G\myparam{W_k}\dotavg{n}}},
\end{flalign}
where \[
G(W_k)=[\nabla \widetilde{f_1}(w_{k,1}), \ldots, \nabla \widetilde{f_n}(w_{k,n})] 
\]
are the stochastic gradient on $n$ nodes based computed with all local samples. 
Because $a^Tb=\frac{1}{2}\myparam{a^2+b^2-(a-b)^2}$, we further obtain:
\begin{flalign}
	\label{eq:step4}
	\nabla f\myparam{W_k\dotavg{n}}^T  \myparam{G\myparam{W_k}\dotavg{n}} = \frac{1}{2} \norm{\nabla f\myparam{W_k\dotavg{n}}} + \frac{1}{2} \norm{G\myparam{W_k}\dotavg{n}} - \frac{1}{2} \norm{\nabla f\myparam{W_k\dotavg{n}} - G\myparam{W_k}\dotavg{n}}.
\end{flalign}
Applying Lipschitzan gradient assumption again, we have:
\begin{flalign}
	\label{eq:step5}
\norm{\nabla f\myparam{W_k\dotavg{n}} - G\myparam{W_k}\dotavg{n}}  &
=\norm{\frac{1}{n}\sum_{i=1}^{n}\nabla f_i\myparam{W_k\dotavg{n}}- \frac{1}{n}\sum_{i=1}^{n}\nabla f_i\myparam{w_{k,i}}}\nonumber\\
\leq&\frac{1}{n} \sum_{i=1}^{n}{\norm{\nabla f_i\myparam{W_k\dotavg{n}} - \nabla f_i\myparam{w_{k,i}}}}
\leq\frac{L^2}{n} \boxed{\sum_{i=1}^{n}{\norm{W_k\dotavg{n} - w_{k,i}}}}.
\end{flalign}
The term in the box is the variance of the model parameters among $n$ nodes. 
Back to formula (\ref{eq:step2}), the last the term can be bounded as:
\begin{flalign}
	\label{eq:step6}
	\mathbb{E}\norm{G(W_k;B_k)\dotavg{n}} 
	=\mathbb{E}\norm{G(W_k;B_k)\dotavg{n}-G(W_k)\dotavg{n}+G(W_k)\dotavg{n}}
	 \leq  \frac{\sigma^2}{M} +\mathbb{E}\norm{G(W_k)\dotavg{n}},
\end{flalign}
where $\sigma^2$ is an upper bound of the variance of stochastic gradient on each node. 
Plugging (\ref{eq:step3}), (\ref{eq:step4}), (\ref{eq:step5}) and (\ref{eq:step6}) into (\ref{eq:step2}), we have:
\begin{flalign}
\label{eq:step7}
	\mathbb{E}f\myparam{W_{k+1}\dotavg{n}} \leq &\mathbb{E}f\myparam{W_{k}\dotavg{n}} -\frac{\gamma_k}{2}\mathbb{E}\norm{\nabla f\myparam{W_k\dotavg{n}}}  - \frac{\gamma_k}{2}\mathbb{E}\norm{G(W_k)\dotavg{n}}\nonumber\\
	+&\frac{L^2\gamma_k}{2n}\mathbb{E}\myrect{\sum_{i=1}^{n}{\norm{W_k\dotavg{n} - w_{k,i}}}}
	+\frac{L\gamma_k^2\sigma^2}{2M}+\frac{L\gamma_k^2}{2}\mathbb{E}\norm{G(W_k)\dotavg{n}}.
\end{flalign}
Suppose $\frac{\gamma_k}{2} > \frac{L\gamma_k^2}{2}$, (\ref{eq:step7}) simplifies to:
\begin{flalign}
\label{eq:step7}
	\mathbb{E}f\myparam{W_{k+1}\dotavg{n}} \leq \mathbb{E}f\myparam{W_{k}\dotavg{n}} -\frac{\gamma_k}{2}\mathbb{E}\norm{\nabla f\myparam{W_k\dotavg{n}}}  	+\frac{L^2\gamma_k}{2n}\mathbb{E}\myrect{\sum_{i=1}^{n}{\norm{W_k\dotavg{n} - w_{k,i}}}}
	+\frac{L\gamma_k^2\sigma^2}{2M},
\end{flalign}
which gives us (\ref{eq:step8}).
\section{Derivation of (\ref{eq:step10})}
We now bound the variance of model parameter among nodes: 
\begin{flalign}
\label{eq:sstt1}
	\mathbb{E}\myrect{\sum_{i=1}^{n}{\norm{W_k\dotavg{n} - w_{k,i}}}}&=\mathbb{E}\myrect{\sum_{i=1}^{n}{\norm{W_k\myparam{\dotavg{n} - \ei{i}}}}}
	=\mathbb{E}\myrect{\sum_{i=1}^{n}{\norm{\myparam{W_{k-1}-\gamma_{k-1}G\myparam{W_{k-1};B_{k-1}}}\myparam{\dotavg{n} - \ei{i}}}}} \nonumber \\
	&=\mathbb{E}\myrect{\sum_{i=1}^{n}{\norm{\myparam{\gamma_{k-1}G\myparam{W_{k-1};B_{k-1}}+ \ldots + \gamma_{l}G\myparam{W_{l};B_{l}}}\myparam{\dotavg{n} - \ei{i}}}}}
\end{flalign}
where $l=p\left\lfloor \frac{k}{p} \right\rfloor $ is the most recent synchronization iteration before $k$.  
Suppose the learning rate in a period is constant, i.e., $\gamma_{k-1} == \gamma_{k-2} == \ldots == \gamma_l$, (\ref{eq:sstt1}) simplifies to: 
\begin{flalign}
\label{eq:sstt2}
	&\mathbb{E}\myrect{\sum_{i=1}^{n}{\norm{W_k\dotavg{n} - w_{k,i}}}}\nonumber\\
	=&\gamma_l^2\mathbb{E}\myrect{\sum_{i=1}^{n}{\norm{\myparam{G\myparam{W_{k-1};B_{k-1}}+ \ldots + G\myparam{W_{l};B_{l}}}\myparam{\dotavg{n} - \ei{i}}}}} \nonumber\\
	=&\gamma_l^2\sum_{i=1}^{n}{ \mathbb{E}\norm{\myparam{G\myparam{W_{k-1};B_{k-1}} - G\myparam{W_{k-1}}  + \ldots + G\myparam{W_{l};B_{l}} - G\myparam{W_{l}} }   \myparam{\dotavg{n} - \ei{i}} }} \nonumber\\ &+  \gamma_l^2\sum_{i=1}^{n}{\mathbb{E}\norm{\myparam{G\myparam{W_{k-1}}+ \ldots + G\myparam{W_{l}}}\myparam{\dotavg{n} - \ei{i}}}} \nonumber \\
	\leq & \gamma_l^2 \sum_{i=1}^{n}\sum_{j=l}^{k-1}\mathbb{E}\norm{\myparam{G\myparam{W_{j};B_{j}} - G\myparam{W_{j}}} \myparam{\dotavg{n} - \ei{i}}} + \gamma_l^2 (k-l) \sum_{i=1}^{n}\sum_{j=l}^{k-1}\mathbb{E}\norm{ G\myparam{W_{j}} \myparam{\dotavg{n} - \ei{i}}}
\end{flalign}
The first term on the right hand side above is the variance of stochastic gradients, which is bounded by:
\begin{flalign}
\label{eq:sstt3}
 \gamma_l^2 \sum_{i=1}^{n}\sum_{j=l}^{k-1}\mathbb{E}\norm{\myparam{G\myparam{W_{j};B_{j}} - G\myparam{W_{j}}} \myparam{\dotavg{n} - \ei{i}}} \leq  \gamma_l^2 \sum_{i=1}^{n}\sum_{j=l}^{k-1}\mathbb{E}\norm{\myparam{G\myparam{W_{j};B_{j}} - G\myparam{W_{j}}}}_F \leq \frac{\gamma_l^2n^2(k-l)\sigma^2}{m}.
\end{flalign}
Here $||\cdot||_F$ represents the Frobenius norm, $m$ is the mini-batch size on each node, and $\sigma^2/m$ is the upper bound of gradient variance on each node. 
The second term on the right hand side of (\ref{eq:sstt2}) is bounded as:
\begin{flalign}
\label{eq:sstt4}
	&\sum_{i=1}^{n}\sum_{j=l}^{k-1}\mathbb{E}\norm{ G\myparam{W_{j}} \myparam{\dotavg{n} - \ei{i}}} \nonumber\\
	\leq & n\sum_{j=l}^{k-1}\mathbb{E}\norm{ G\myparam{W_{j}} }_F= n\sum_{j=l}^{k-1}\sum_{s=1}^{n}\mathbb{E}\norm{ \nabla f_s(w_{j,s}) }\nonumber \\ = & n\sum_{j=l}^{k-1}\sum_{s=1}^{n}\mathbb{E}\norm{ \nabla f_s(w_{j,s}) -\nabla f(w_{j,s}) + \nabla f(w_{j,s})  -\nabla f\myparam{W_j\dotavg{n}} + \nabla f\myparam{W_j\dotavg{n}} } \nonumber \\
	\leq & 3n\sum_{j=l}^{k-1}\sum_{s=1}^{n}\mathbb{E}\norm{ \nabla f_s(w_{j,s}) -\nabla f(w_{j,s})} + 3n\sum_{j=l}^{k-1}\sum_{s=1}^{n}\mathbb{E}\norm{\nabla f(w_{j,s})  -\nabla f\myparam{W_j\dotavg{n}}} +  3n\sum_{j=l}^{k-1}\sum_{s=1}^{n}\mathbb{E}\norm{f\myparam{W_j\dotavg{n}} } \nonumber\\
	\leq & 3n^2(k-l)\varsigma^2 + 3nL^2\cdot \sum_{j=l}^{k-1} \mathbb{E}\myrect{\sum_{i=1}^{n}{\norm{W_j\dotavg{n} - w_{j,i}}}} + 3n^2\sum_{j=l}^{k-1}\mathbb{E}\norm{f\myparam{W_j\dotavg{n}} }. 
\end{flalign}
Here, $\varsigma^2$ is the upper bound of variance of gradients across nodes, and the last step is based on Lipschitzan gradient assumption. 
Plugging (\ref{eq:sstt4}) and (\ref{eq:sstt3}) into (\ref{eq:sstt2}), we can obtain:
\begin{flalign}
	 \Var{W_k}=&\mathbb{E}\myrect{\frac{1}{n}\sum_{i=1}^{n}{\norm{W_k\dotavg{n} - w_{k,i}}}} \nonumber \\ \leq & 
	 \frac{\gamma_l^2n(k-l)\sigma^2}{m} + 3 \gamma_l^2 n(k-l)^2\varsigma^2 + 3\gamma_l^2n(k-l)L^2 \sum_{j=l}^{k-1}\Var{W_j}  + 3\gamma_l^2n(k-l)\sum_{j=l}^{k-1}\mathbb{E}\norm{f\myparam{W_j\dotavg{n}} }
\end{flalign}
Summing up $\Var{W_k}$ for $k \in [l, l+p)$, we have:
\begin{flalign}
	\sum_{k=l}^{l+p-1}{\Var{W_k}} \leq  \frac{\gamma_l^2np^2\sigma^2}{m} + 3 \gamma_l^2 np^3\varsigma^2 + 3\gamma_l^2np^2L^2 \sum_{k=l}^{l+p}{\Var{W_k}} + 3\gamma_l^2np^2\sum_{j=l}^{k-1}\mathbb{E}\norm{f\myparam{W_j\dotavg{n}} }
\end{flalign}
It follows that
\begin{flalign}
\label{eq:sstt5}
	\sum_{k=l}^{l+p-1}{\Var{W_k}} \leq  \frac{1}{1-3\gamma_l^2np^2L^2 } 
\myparam{\frac{\gamma_l^2np^2\sigma^2}{m} + 3 \gamma_l^2 np^3\varsigma^2 +  3\gamma_l^2np^2\sum_{j=l}^{k-1}\mathbb{E}\norm{f\myparam{W_j\dotavg{n}} }}
\end{flalign}
and 
\begin{flalign}
\label{eq:vtbound}
	V_t=\frac{1}{p}\sum_{k=pt}^{p(t+1)-1}{\Var{W_k}} \leq  \frac{1}{1-3\gamma_{pt}^2np^2L^2 } 
\myparam{\frac{\gamma_{pt}^2np\sigma^2}{m} + 3 \gamma_{pt}^2 np^2\varsigma^2 +  3\gamma_{pt}^2np\sum_{j=l}^{k-1}\mathbb{E}\norm{f\myparam{W_j\dotavg{n}} }}
\end{flalign}
Suppose $\gamma_k=\gamma$ for all $k$'s, averaging  $\Var{W_k}$ for $k \in [0, K)$, we have:
\begin{flalign}
	\mathbb{E} \myrect{\frac{1}{K}\sum_{k=0}^{K-1}\Var{W_k} } \leq    \frac{\gamma^2np \myparam{\frac{\sigma^2}{m} + 3p\varsigma^2}}{1-3\gamma^2np^2L^2 } + 
	 \frac{3\gamma^2np}{1-3\gamma^2np^2L^2}\cdot\frac{1}{K}\sum_{k=0}^{K-1}\mathbb{E}\norm{\nabla f\myparam{W_{k}\dotavg{n}}}, 
\end{flalign}
This gives us (\ref{eq:step10}) with $C_1=\frac{\sigma^2}{m} + 3p\varsigma^2$.


\newpage
\section{The Advantage of Periodic Parameter Averaging SGD in Generalization Performance}

Smith {\em et al.}~\cite{l.2018a} recently gives an explanation of generalization performance  of deep neural networks from a Bayesian perspective. 
 We briefly summarize their main idea here to facilitate our discussion. 
 Readers can refer to~\cite{l.2018a} for more details.  
 To compare the quality of different minima in non-convex functions, they define the {\em Bayesian evidence} in favor of a minimum as the integral of the posterior over the {\em bowl of attraction}  
  that  surrounds that minimum. 
 A stronger evidence indicates the minimum is deeper and flatter, and thus  has better test accuracy. 
Based on this interpretation, the authors make a connection between SGD  that 
 finds minima of differentiable functions and the overdamped Langevin equation: 
\begin{equation}
\label{eq:lange}
	\frac{dw}{dt}=-\frac{df(w)}{dw}+\eta(t)
\end{equation}
which samples parameter values from the Bayesian posterior~\cite{6796869}.  
 Here $\eta(t)$ is a Gaussian noise with $\mathbb{E}[\eta(t)]=0$ and corelation function $\mathbb{E}[\eta(t)\eta(t')]=2TI\delta(t-t')$ where $I$ is identity matrix, $T$ is the {\em temperature}, and $\delta$ is the Dirac delta function. 
The discretization of the above Langevin equation is: 
 \begin{equation}
 \label{eq:langint}
 	\Delta w =  -\gamma \nabla f(w) + \int_0^{\gamma}\eta(t)dt.
 \end{equation}
Comparing the above equation with one step in SGD:
 \begin{equation}
 \label{eq:sgdupdate}
	\Delta w  = - \gamma \nabla f(w) + \gamma \myparam{  \nabla f(w) -  \nabla \widetilde{f}(w) },
\end{equation}
we can see that SGD will behave similar to Bayesian sampling if the gradient noise $\gamma\myparam{\nabla \widetilde{f}(w) -  \nabla f(w)}$ is close to the Gaussian noise $\int_0^{\gamma}\eta(t)dt$.  
An important property of Langevin dynamics is that they sample a parameter vector belonging to a local minimum with a probability proportional to the integral of the posterior over the bowl of attraction surrounding that minimum~\cite{Welling:2011:BLV:3104482.3104568}\cite{l.2018a}\cite{NIPS2017_6664}. 
Recall that the integral of posterior around a minimum is the Bayesian evidence in favor of that minimum. 
The property means that the Langevin dynamics tends to sample minimum with better  accuracy. 
Therefore, the authors claim that SGD will reach a minimum  with 
a  better  accuracy  if it has gradient noise similar to the Gaussian noise in the Langevin dynamics.  

\subsection{Gradient Noise in Vanilla SGD}
Smith {\em et al.}~\cite{l.2018a} derive the covariance matrix of the gradient noise in mini-batch SGD as
\begin{flalign}
\label{eq:covgrad}
	&\Covariance{\gamma\myparam{ \nabla f(w) -  \nabla \widetilde{f}(w)}, \gamma\myparam{ \nabla f(w) -  \nabla \widetilde{f}(w)}} \nonumber \\
	= &  \gamma^2 \Covariance{ \nabla \widetilde{f}(w),  \nabla \widetilde{f}(w)} = \gamma^2 \myparam{\frac{1}{M}-\frac{1}{N}}Q(w)
\end{flalign}
where $N$ is the total number of samples, $M$ is the mini-batch size and 
\begin{equation}
\label{eq:qw1}
	Q(w)=\frac{1}{N}\sum_{i=1}^{N}\nabla F_i(w)\nabla F_i^T(w) 
\end{equation}
describes the gradient covariance. 
Comparing (\ref{eq:covgrad}) with the covariance matrix of noise in (\ref{eq:langint}):
\begin{flalign}
\label{eq:coveta}
	&\Covariance{ \int_0^{\gamma}\eta(t)dt,  \int_0^{\gamma}\eta(t)dt} = 2TI\gamma,
\end{flalign}
the authors 
claim that one should keep $\gamma^2 \myparam{\frac{1}{M}-\frac{1}{N}} \propto \gamma$ to achieve good  
accuracy  with large $M$. 
This result implies the {\em linear scaling rule}~\cite{DBLP:journals/corr/GoyalDGNWKTJH17} for large-batch SGD, i.e., the learning rate should increase proportionally to the mini-batch size. 
Their conclusion is consistent with the convergence analysis of mini-batch SGD~\cite{Dekel:2012:ODO:2503308.2188391} and is supported by recent empirical studies~\cite{DBLP:journals/corr/GoyalDGNWKTJH17}. 

\subsection{Gradient Noise in Periodic Averaging SGD}
To show the advantage of periodic averaging SGD, we now derive the noise in periodic averaging SGD. 
We first show
\begin{equation}
\label{eq:limexpect}
	\lim_{\gamma\rightarrow 0}\mathbb{E}[h(W;B)]= \overrightarrow{\bf 0}
\end{equation}
Note that even though the noise in vanilla SGD has expected value of zero, (\ref{eq:sgdupdate}) is a biased simulation of (\ref{eq:lange}) when $\gamma>0$~\cite{Wibisono2018SamplingAO}. 
Therefore, it is enough to show the expected noise when $\gamma \rightarrow 0$. 
According to Algorithm~\ref{alg1}, we have
\begin{flalign}
\label{eq:limeh}
	&\lim_{\gamma\rightarrow 0}\mathbb{E}[h(W;B)] = \lim_{\gamma\rightarrow 0}\mathbb{E}\myrect{ \nabla f(w)-G(W;B)\dotavg{n}} \nonumber \\ 
	=& \lim_{\gamma\rightarrow 0}\mathbb{E} \myrect{ \nabla f\myparam{w_{pt}-\frac{\gamma}{n} \sum_{i=1}^{n}\myparam{\nabla \widetilde{f_i}(w_{pt,i}) +  \ldots \nabla \widetilde{f_i}(w_{pt+s,i})}}-  
	 \frac{1}{n} \sum_{i=1}^{n} \nabla f\myparam{w_{pt,i} - \gamma\myparam{\nabla \widetilde{f_i}(w_{pt,i})  + \ldots \nabla \widetilde{f_i}(w_{pt+s,i})}} } \nonumber\\
	 =&\frac{1}{n}\sum_{i=1}^{n}\lim_{\gamma\rightarrow 0}\mathbb{E} \myrect{ \nabla f\myparam{w_{pt}-\frac{\gamma}{n} \sum_{i=1}^{n}\myparam{\nabla \widetilde{f_i}(w_{pt,i}) +  \ldots \nabla \widetilde{f_i}(w_{pt+s,i})}} -\nabla f\myparam{w_{pt,i} - \gamma\myparam{\nabla \widetilde{f_i}(w_{pt,i})  + \ldots \nabla \widetilde{f_i}(w_{pt+s,i})}}}
\end{flalign}
where $w_{pt,i}$ is the model parameters in iteration $pt$ on node $i$, and $s\leq p$ is the number of iterations since iteration $pt$ when last synchronization happens. 
According the Lipschitz continuous gradient assumption, we have:  
\begin{flalign}
	&\lim_{\gamma \rightarrow 0}\mathbb{E}\normb{\nabla f\myparam{w_{pt}-\frac{\gamma}{n} \sum_{i=1}^{n}\myparam{\nabla \widetilde{f_i}(w_{pt,i}) +  \ldots \nabla \widetilde{f_i}(w_{pt+s,i})}} -\nabla f\myparam{w_{pt,i} - \gamma\myparam{\nabla \widetilde{f_i}(w_{pt,i})  + \ldots \nabla \widetilde{f_i}(w_{pt+s,i})}}} \nonumber\\
	\leq &\lim_{\gamma \rightarrow 0} L^2\gamma^2 \normb{\frac{1}{n} \sum_{i=1}^{n}\myparam{\nabla \widetilde{f_i}(w_{pt,i}) +  \ldots \nabla \widetilde{f_i}(w_{pt+s,i})} - \myparam{\nabla \widetilde{f_i}(w_{pt,i})  + \ldots \nabla \widetilde{f_i}(w_{pt+s,i})}} \nonumber \\
	= & 0
\end{flalign}
Thus, 
\begin{flalign}
\label{eq:tmp1111}
	\lim_{\gamma \rightarrow 0}\mathbb{E} \myrect {\nabla f\myparam{w_{pt}-\frac{\gamma}{n} \sum_{i=1}^{n}\myparam{\nabla \widetilde{f_i}(w_{pt,i}) +  \ldots \nabla \widetilde{f_i}(w_{pt+s,i})}} -\nabla f\myparam{w_{pt,i} - \gamma\myparam{\nabla \widetilde{f_i}(w_{pt,i})  + \ldots \nabla \widetilde{f_i}(w_{pt+s,i})}}} = \overrightarrow{\bf 0}
\end{flalign}
Plugging (\ref{eq:tmp1111}) into (\ref{eq:limeh}), we can see $\lim_{\gamma\rightarrow 0}\mathbb{E}[h(W;B)]= \overrightarrow{\bf 0}$. 
It is apparent that the above derivation can be generalized to adaptive periodic averaging with non-constant averaging period. 
Therefore,  (\ref{eq:limexpect}) is also valid in our ADPSGD. 


\noindent
Next, we compute the covariance of the noise:
\begin{flalign}
\Cov [\gamma h(W;B), \gamma h(W;B)] = \gamma^2 \Covariance{G(W;B)\dotavg{n},G(W;B)\dotavg{n}}	 
 = \frac{\gamma^2}{n^2}\Covariance{\sum_{j=1}^{n}\nabla \widetilde{f_j}(w_j;B_j),\sum_{j=1}^{n}\nabla \widetilde{f_j}(w_j;B_j)}
\end{flalign}
where $w_j$ and $B_j$ is the model parameters and the mini-batch on node $j$. 
Assuming the sampling of training data on each node is independent, i.e.,
\[
\Covariance{\nabla \widetilde{f_i}(w_i;B_i),\nabla \widetilde{f_j}(w_j;B_j)}=0, \text{ if $j\neq i$},
\]
we have:
\begin{flalign}
\label{eq:45s1}
	\Cov [h(W;B), h(W;B)]  = \frac{\gamma^2}{n}\sum_{j=1}^{n}\Covariance{\nabla\widetilde{f_j}(w_j;B_j), \nabla \widetilde{f_j}(w_j;B_j)}
\end{flalign}
We define a random variable $s_i$ as 
\begin{flalign}
	s_i=\begin{cases}
		1 &,\; \text{ if sample $i$ is selected}\\
		0 &,\; \text{ if sample $i$ is not selected}
	\end{cases}
\end{flalign}
Then, $\nabla\widetilde{f_j}(w_j;B_j)$ can be represented as
\begin{equation}
	\nabla\widetilde{f_j}(w_j;B_j) = \frac{1}{M}\sum_{i=1}^{N}\nabla F_i(w_j)s_i
\end{equation}
where $N$ is the total number of training data and $M$ is the mini-batch size. 
We know $w=\frac{1}{N}\sum_{j=1}^{N}w_j$, and $w_j\neq w$ for most iterations (except the iteration right after synchronization). 
%Suppose the last synchronization happens in iteration $j'$, the value of $w_j$ depends on the stochastic model parameter updates between iteration $j'$ and $j$. 
%There are a finite number of possible $w_j$ because there are a finite number of combinations of sampling the training data between iteration $j'$ and $j$. 
Without loss of generality, 
we can simply consider $w_j$ as a random variable with probability density function $\rho$. 
Then, $\nabla\widetilde{f_j}(w_j;B_j)$ can be further represented as
\begin{equation}
	\nabla\widetilde{f_j}(w_j;B_j) = \frac{1}{M}\int_\omega \sum_{i=1}^{N}\nabla F_i(\omega)s_i \delta(\omega-w_j)d\omega
\end{equation} 
It follows that 
\begin{flalign}
	\Covariance{\nabla\widetilde{f_j}(w_j;B_j), \nabla \widetilde{f_j}(w_j;B_j)}=&\frac{1}{M^2}\Covariance{\int_\omega \sum_{i=1}^{N}\nabla F_i(\omega)s_i \delta(\omega-w_j)d\omega,\int_\omega \sum_{i=1}^{N}\nabla F_i(\omega)s_i \delta(\omega-w_j)d\omega} 
	\nonumber\\
	=&\frac{1}{M^2} \int_\omega d\omega \int_\omega' d\omega'  \Covariance{\sum_{i=1}^{N}\nabla F_i(\omega)s_i\delta(\omega-w_j), \sum_{i=1}^{N}\nabla F_i(\omega')s_i\delta(\omega'-w_j)}
	\end{flalign}
Assume the stochastic gradients at different points are independent, i.e.,
\begin{flalign}
	\Covariance{\sum_{i=1}^{N}\nabla F_i(\omega)s_i\delta(\omega-w_j), \sum_{i=1}^{N}\nabla F_i(\omega')s_i\delta(\omega'-w_j)}=0, \text{ if $\omega\neq \omega'$}
\end{flalign}
Then, 
\begin{flalign}
	\Covariance{\nabla\widetilde{f_j}(w_j;B_j), \nabla \widetilde{f_j}(w_j;B_j)}=&\frac{1}{M^2} \int_\omega d\omega   \Covariance{\sum_{i=1}^{N}\nabla F_i(\omega)s_i\delta(\omega-w_j), \sum_{i=1}^{N}\nabla F_i(\omega)s_i\delta(\omega-w_j)} \nonumber \\
	=& \frac{1}{M^2} \int_\omega d\omega \sum_{i=1}^{N}\sum_{j=1}^{N} \Covariance{\nabla F_i(\omega)s_i \delta(\omega-w_j), \nabla F_j(\omega)s_j\delta(\omega-w_j)}.
\end{flalign}
And because the sampling of training data is also independent, i.e.,
\[
\Covariance{\nabla F_i(\omega)s_i\delta(\omega-w_j), \nabla F_j(\omega)s_j\delta(\omega-w_j)}=0, \text{ if $i\neq j$}
\]
we have: 
\begin{flalign}
\label{eq:45s2}
	\Covariance{\nabla\widetilde{f_j}(w_j;B_j), \nabla \widetilde{f_j}(w_j;B_j)}=&\frac{1}{M^2}\int_\omega d\omega \sum_{i=1}^{N}\Covariance{\nabla F_i(\omega)s_i \delta(\omega-w_j), \nabla F_i(\omega)s_i \delta(\omega-w_j)}\nonumber\\
	=&\frac{1}{M^2}\int_\omega d\omega \sum_{i=1}^{N}\nabla F_i(\omega)^T\nabla F_i(\omega)\Covariance{s_i \delta(\omega-w_j),s_i \delta(\omega-w_j)} \nonumber\\
	=&\frac{1}{M^2}\int_\omega d\omega \sum_{i=1}^{N}\nabla F_i(\omega)^T\nabla F_i(\omega)\myparam{\mathbb{E}[s_i^2 \delta^2(\omega-w_j)]-\mathbb{E}^2[s_i \delta(\omega-w_j)]}
\end{flalign}
Because $w_j$ depends on the stochastic parameter updates before iteration $j$ and $s_j$ is the sampling in iteration $j$, it is reasonable to assume $s_i$ and $w_j$ are independent. Thus,
\begin{equation}
\label{eq:45s3}
	\mathbb{E}[s_i^2 \delta^2(\omega-w_j)]-\mathbb{E}^2[s_i \delta(\omega-w_j)]=\mathbb{E}[s_i^2] \mathbb{E}[\delta^2(\omega-w_j)]-\mathbb{E}^2[s_i] \mathbb{E}^2[\delta(\omega-w_j)]
\end{equation}
Plugging (\ref{eq:45s3}) into (\ref{eq:45s2}), and (\ref{eq:45s2}) into (\ref{eq:45s1}), we can get:
\begin{flalign}
\label{eq:45s4}
	\Cov [h(W;B), h(W;B)]=\frac{\gamma^2}{nM^2}\sum_{j=1}^n\int_\omega d\omega \sum_{i=1}^{N}\nabla F_i(\omega)^T\nabla F_i(\omega)\myparam{\mathbb{E}[s_i^2] \mathbb{E}[\delta^2(\omega-w_j)]-\mathbb{E}^2[s_i] \mathbb{E}^2[\delta(\omega-w_j)]}
\end{flalign}
Note that we have not assumed any specific distribution for $s_i$ and $w_j$ so far. 
We now assume the sampling of training data is uniform. 
It is easy to see $\mathbb{E}[s_i]=M/N$ and $\mathbb{E}[s_i^2]=M/N$. 
Also, because $w_j$ has probability density function $\rho$, we have:
\begin{flalign}
\label{eq:45s5}
	&\Cov [h(W;B), h(W;B)]=\frac{\gamma^2}{nM^2}\sum_{j=1}^n\int_\omega d\omega \sum_{i=1}^{N}\nabla F_i(\omega)^T\nabla F_i(\omega)\myparam{\frac{M}{N} \rho(\omega)-\frac{M^2}{N^2} \rho^2(\omega)} \nonumber\\
%	=& \frac{\gamma^2}{nM^2}\sum_{j=1}^n\myparam{\frac{M}{N} \rho_j(\omega)-\frac{M^2}{N^2} \rho_j^2(\omega)}
% \int_\omega d\omega \sum_{i=1}^{N}\nabla F_i(\omega)^T\nabla F_i(\omega)
% \nonumber\\ = &
=&  \frac{\gamma^2}{M^2}\int_\omega d\omega\myparam{\frac{M}{N} \rho(\omega)-\frac{M^2}{N^2} \rho(w_j)+ \frac{M^2}{N^2} \rho(w_j)-\frac{M^2}{N^2} \rho^2(\omega)}
 \sum_{i=1}^{N}\nabla F_i(\omega)^T\nabla F_i(\omega) \nonumber\\
 =& \gamma^2\myparam{\frac{1}{M}-\frac{1}{N}}\int_\omega d\omega  \rho(\omega)\frac{1}{N}\sum_{i=1}^{N}\nabla F_i(\omega)^T\nabla F_i(\omega) + \gamma^2 \frac{1}{N}\int_\omega d\omega(\rho(\omega)-\rho^2(\omega))\frac{1}{N}\sum_{i=1}^{N}\nabla F_i(\omega)^T\nabla F_i(\omega)
 \end{flalign}
which gives us:
\begin{flalign}
\label{eq:covper_main}
\Cov [\gamma h(W;B&), \gamma h(W;B)] = \gamma^2\Covariance{G(W;B)\dotavg{n},G(W;B)\dotavg{n}}	\nonumber \\
=&\gamma^2 \myparam{\frac{1}{M}-\frac{1}{N}}D_1(W) +  \frac{\gamma^2}{N} D_2(W)
\end{flalign}
where 
\vspace{-1em}
\begin{flalign}
\label{eq:qw2}
	D_1(W)=\int_\omega d\omega  \rho(\omega)Q(\omega)
	\end{flalign}
	and \begin{flalign}
	D_2(W)=\int_\omega d\omega \myparam{ \rho(\omega)- \rho^2(\omega)}Q(\omega)	
\end{flalign}
Here, $\omega \sim \Omega$ is a distribution of the model parameters, with probability density function $\rho$. 
%The distribution depends on the stochastic parameter updates on each node since last synchronization. 
%Because the sampling of training data is usually assumed to be uniform, $\omega \sim \Omega$ is also uniform if the stochastic gradients  computed with different mini-batches lead to distinct model parameters. 
%The $\varrho$ in the above equation is the probability of one possible parameter value. 
%Note that (\ref{eq:noiseofvanilla}) is a special case of  (\ref{eq:covgrad}). 
When the model parameters are synchronized in every iteration, the only value of $\omega$ is $w=W\dotavg{n}$ and $\rho(w)=1$. 
We can see that $D_1(W)=Q(w), D_2(W)=0$, and (\ref{eq:covper_main}) becomes the same as (\ref{eq:covgrad}). 

Suppose $Q(\omega)\approx Q(w)$ for $\omega$ near $w$, the first term on the right hand side of  (\ref{eq:covper_main}) will be close to (\ref{eq:covgrad}). 
The second term on the right hand side of  (\ref{eq:covper_main}) adds extra noise to the training process.  
Thus, periodic averaging has higher potential to escape sharp minimum than vanilla SGD. 


%Because the sampling of training data is uniform, $w_j$ is uniform in the set of all its possible values if stochastic gradients computed with different mini-batches leads to distinct model parameters. 
%In this case, the probability density function is constant: 
%\begin{equation}
%	\rho_j(w_j)=\varrho, \forall j\; \text{ , if $w_j$ is in the set of possible parameter values}
%\end{equation} 
%The value of $\varrho$ depends on the averaging period $p$. 
%The larger the averaging period $p$, the more possible values of $w_j$ and thus the smaller $\varrho$.  
%Based on this assumption, we further simplify (\ref{eq:45s5}) to 
%\begin{flalign}
%\label{eq:tmpeeeee}
%	\Cov [h(W;B), h(W;B)]=&\frac{\gamma^2}{M^2}\myparam{\frac{M}{N}\varrho -\frac{M^2}{N^2} \varrho^2}
% \cdot \int_\omega d\omega \sum_{i=1}^{N}\nabla F_i(\omega)^T\nabla F_i(\omega)\nonumber\\
% =&\gamma^2\myparam{\frac{1}{M} -\frac{\varrho}{N} } Q'(W) 
% \end{flalign}
%where 
%\begin{equation}
%	Q'(W)=\frac{\varrho}{N} \int_\omega d\omega \sum_{i=1}^{N}\nabla F_i(\omega)^T\nabla F_i(\omega)
%	\end{equation}
%This gives us (\ref{eq:covper}). 
%Note that $\int_{\omega}\rho_j(\omega) d\omega=1$, we can consider $Q'(W)$ as a constant if $\nabla F_i(\omega)$ at different $\omega$ have similar magnitude. 
%Because a larger $p$ leads to a smaller $\varrho$, it also leads to a larger value of the second term on the right hand side of (\ref{eq:tmpeeeee}).

%Now, let us compare period averaging SGD with vanilla mini-batch SGD. 
%Suppose vanilla SGD achieves best accuracy with batch size $m$ and learning rate $\gamma$, and we want to scale the computation to $n$ nodes (i.e., total mini-batch size becomes $M=mn$). 
%The covariance in (\ref{eq:covgrad}) suggests increasing the learning rate to $n\gamma$ to maintain the noise scale of small-batch SGD; however, a large learning rate leads to large discretization error in (\ref{eq:sgdupdate}) for simulating (\ref{eq:lange})~\cite{l.2018a}. 
%Also, the linear scaling rule is applicable only if $M \ll N$ because when $M \rightarrow N$ the SGD becomes gradient descent and a well-known upper bound of the learning rate for gradient descent is $1/L$ where $L$ is the Lipschitz constant of the objective function~\cite{doi:10.1137/070704277}. 
%These indicate that we cannot simply increase the learning rate to achieve good  accuracy 
%for large-batch SGD.  
%In fact, the linear scaling rule cannot  generalize  to CIFAR-10~\cite{NIPS2017_6770} dataset and AlexNet on ImageNet dataset~\cite{NIPS2017_6770, DBLP:journals/corr/abs-1708-03888, DBLP:journals/corr/abs-1805-07898}. 
%Now,  if we let the nodes synchronize less frequently, the second term on the right hand side of  (\ref{eq:tmpeeeee}) will compensate for the decrease of $\myparam{\frac{1}{M}-\frac{1}{N}}$. 
%Therefore, we can keep the noise scale of small-batch SGD with smaller increase of the learning rate compared with vanilla SGD.  


\newpage
\section{Results on ImageNet}

\begin{figure*}
	\centering
	\subfloat[Training Loss]{
	\includegraphics[scale=0.33]{figures/resnet50_imagenet_loss.pdf}
	}
	\subfloat[1-Crop Validation Accuracy]{
	\includegraphics[scale=0.33]{figures/resnet50_imagenet_accuracy.pdf}
			\label{fig:imagenetresnetacc}
	}
	\subfloat[Execution Time]{
	\includegraphics[scale=0.34]{figures/resnet50_imagenet_time.pdf}
			\label{fig:imagenetresnettime}
	}
		\vspace{-0.5em}
	\caption{Training ResNet50 on ImageNet with 16 GPUs}
		\label{fig:imagenetresnet}
\end{figure*}

ILSVRC 2012 (ImageNet)~\cite{imagenet_cvpr09} is a much larger dataset than CIFAR-10. 
 There are a total of 1,281,167 images in 1000 classes for training, and 50,000 images for validation. 
 The images vary in dimensions and resolution. The average resolution is 469x387 pixels. 
Normally the images are resized to 256x256 pixels for neural networks.  


We train a ResNet50~\cite{DBLP:journals/corr/HeZRS15} on ILSVRC 2012. 
%The mini-batch size on each node is 128, and the total mini-batch size on 16 nodes is 2048. 
We apply the {\em linear scaling rule} and the {\em gradual warmup} techniques proposed in 
literature~\cite{DBLP:journals/corr/GoyalDGNWKTJH17} for all versions of SGD in our experiments. 
Specifically, the first $8$ epochs are warmup -- the learning rate is initialized to $0.1$ and is  
increased by $0.1$ in each epoch until the epoch $8$. 
Starting from the epoch $8$, the learning rate is fixed at $0.8$ until epoch $30$ when the learning rate is decreased to $0.08$. 
At epoch $60$, the learning rate is further decreased to $0.008$. 
The total number of epochs is $90$. 
For ADPSGD and CPSGD, the periodic averaging is applied after the warmup phase (i.e., the first $8$ epochs in ADPSGD and CPSGD are the same as in FULLSGD).  
For ADPSGD, Algorithm~\ref{alg2} is applied with $p_{init}=4$, $K_s=0.2K$ where $K$ is the total number of training iterations. 
For QSGD, the gradient quantization is also started after the warmup phase. 


Figure~\ref{fig:imagenetresnet} shows the training loss and the top-1 validation accuracy achieved by different versions. (We evaluate the accuracy on the validation data in ILSVRC 2012).  
The validation images are resize to $256\times 256$ in which the center $224\times 224$ crop are used for validation. (This is the same as in the original ResNet paper~\cite{DBLP:journals/corr/HeZRS15}). 
We can see that our ADPSGD achieves smaller training loss and higher validation accuracy than CPSGD with $p=8$. 
The average averaging period in our ADPSGD is $10.55$, which means that our ADPSGD achieves better convergence than CPSGD while requiring  less communication. 
Compared with QSGD, our ADPSGD also achieves  smaller training loss and higher validation accuracy while requiring less communication. 
Compared with FULLSGD, our ADSGD achieves slightly larger training loss but almost the same test accuracy. 
The dashed line in Figure~\ref{fig:imagenetresnetacc} is the accuracy achieved by small-batch SGD -- we train ResNet50 with batch size $256$ and initial learning rate $0.1$, and the best accuracy we achieved is $75.458\%$. 
The validation error (i.e., $1-accuracy$) reported in the original ResNet paper~\cite{DBLP:journals/corr/HeZRS15} is $24.7\%$, which is close to the accuracy we achieved, so we use $75.458\%$ as the baseline accuracy for comparison. 
We can see in Figure~\ref{fig:imagenetresnetacc} that the best accuracy achieved by our ADPSGD is quite close to the baseline. 

Figure~\ref{fig:imagenetresnettime} shows the execution time of different versions. 
About $25\%$ of total execution time of FULLSGD is spent on communication with 100Gbps connection, and the ratio increases to $56\%$ with 10Gbps connection. 
Our ADPSGD effectively reduces the communication overhead and achieves $1.27x$ and $1.95$x speedups against  
FULLSGD with 100Gbps and 10Gbps connections,  respectively. 
The speedups of 16-node ADPSGD over single-node vanilla SGD are $15.75$x and $14.94$x with 100Gbps and 10Gbps connections respectively, indicating that our ADPSGD achieves linear speedup across 16 nodes. 



